Simultaneous Multiple-Prompt Guided Generation Using Differentiable Optimal Transport

Recent advances in deep learning, such as powerful generative models and joint text-image embeddings, have provided the computational creativity community with new tools, opening new perspectives for artistic pursuits. Text-to-image synthesis approaches that operate by generating images from text cues provide a case in point. These images are generated with a latent vector that is progressively refined to agree with text cues. To do so, patches are sampled within the generated image, and compared with the text prompts in the common text-image embedding space; The latent vector is then updated, using gradient descent, to reduce the mean (average) distance between these patches and text cues. While this approach provides artists with ample freedom to customize the overall appearance of images, through their choice in generative models, the reliance on a simple criterion (mean of distances) often causes mode collapse: The entire image is drawn to the average of all text cues, thereby losing their diversity. To address this issue, we propose using matching techniques found in the optimal transport (OT) literature, resulting in images that are able to reflect faithfully a wide diversity of prompts. We provide numerous illustrations showing that OT avoids some of the pitfalls arising from estimating vectors with mean distances, and demonstrate the capacity of our proposed method to perform better in experiments, qualitatively and quantitatively.

==> contents/6.acknowledgement.tex <==
\section{acknowledgement}

The authors thanks Yujin Tang, Jerry Li, Mathieu Blondel for their valuable comments.

==> contents/__latexindent_temp.tex <==

\section{Foundations and Motivations}

In this section, we give a brief overview two important foundations in our work,
namely \textbf{Prompt-guided Image Geneartion} and \textbf{Differentiable Optimal Transport}.
Although they seem to be unrelated, combinining them is important in address issues we observed in existing methods,
as we furthermore discuss the \textbf{Motivation of Our Work}.
As these issues are dicussed in the framing of our method, they should serve as a good foundations for our methodology dicussed later.

\subsection{Prompt Guided Image Generation}

% talk about 
In the recent wave of computational creativity, one notable trend is to guding the image generation using natural language as prompts.
Such computational tools are essentially text-to-painting synthesis tools that allow artists to specify what to be painted by a generative model using prompts in natural languages.
This text-driven generation largely revolutionlizes the computational generation of artworks,
which can be seen in the online currated collections~\cite{snell2021,murdock}.

The advacnes are made possible by combining two advances in deep learning:
\begin{enumerate}
    \item \textbf{Powerful image generative models}. 
        Such models include recent Generative Adversarial Networks (GANs)~\cite{karras2019style,karras2020analyzing,karras2021alias}, 
        Variational Autoencoder~\cite{van2017neural} 
        and Diffusion Models~\cite{ho2020denoising,song2020denoising,nichol2021improved,dhariwal2021diffusion},
        that can produce images with high fidelity and diversity.
        Their capacity has become \todowritingintext{cite anime/other gaugan}.
    \item \textbf{Modeling images and natural languages jointly}.
        Such an idea has never been completely new~\cite{thomee2016yfcc100m,li2017learning},
        but only with recent advances on generality in natural languages modeling~\cite{raffel2019exploring,brown2020language}
        make it possble to model images and natural languages jointly so the generaltiy is well to eliminate the need for task-specific fine-tuning, as shown in CLIP~\cite{radford2021learning}.
\end{enumerate}



% next: formulated 

\subsection{Differentiable Optimal Transport}


\subsection{Motivation of Our Work}


\subsection{Below are uncleaned parts}

\subsection{Prompt Guided Image Generation}

\todowriting{Prompt Guided Image Generation. (a) fix the citation of referred works. (2) Add related works form neurips 
creativity workshop 2021 to citation and discuss them.}

% Generative Adversarial Networks (GANs)~\cite{karras2019style,karras2020analyzing,karras2021alias}, 
% Variational Autoencoder~\cite{van2017neural} 
% Diffusion Models~\cite{ho2020denoising,song2020denoising,nichol2021improved,dhariwal2021diffusion}


% https://ott-jax.readthedocs.io/en/stable/_autosummary/ott.core.sinkhorn.sinkhorn.html
% ^ sinkorn with diffetiation

% for OT, we will need to use the notation in comptuational optima ltransport
% Tangent measure ... Radon Measure....

This is enabled by the use of pre-trained CLIP~\cite{radford2021learning},
which provides two encoders for text and image respectively that are jointly trained, 
such that the encoded text and images are in the same, comparable space with Cosine Distance. 
In doing so, 
the difference between the image and the user-specific prompt as a text can be calculated and leveraged as a guidence to adjust image.
As the encoders in CLIP are differentiable, such guidence is often materialized as a greadent on the image 
which is the output of  a differtiable generative model so the  gradient can be further back-propagated and the adjustment is done iteratively using Gradient Descent.
The choice of such generative model can vary.

In one direction, CLIP is used to guide good performing unconditional GANs, such as guiding BigGAN (code~\cite{wang2021bigsleep}, reddit discussion), VQGAN (guid~e\cite{samburtonking2021introduction}), siren (an implicit model) (code~\cite{wang2021deepdaze}), or a GAN with genetic algorithm-generated latent space (paper). In this direction, GANs are unconditional (except for being conditioned on the language prompt as interpreted by CLIP). 
CLIP is also used guide the conditional generation using GANs. Here condition means information other than language prompt, such as the original image in the application of image editing. In this direction, StyleCLIP(code, paper) proposes to guide attribute manipulation of StyleGAN2.

In another direction, CLIP can be used on Diffusion models~\cite{ho2020denoising,song2020denoising,nichol2021improved,dhariwal2021diffusion} too.
\todowriting{Adding a quick overview of diffusion models. Also refer to such CLIP + Diffution works and discuss them}.

\subsection{Differentiable Optimal Transport}

\todowriting{Differentiable Optimal Transport}

% Some refer to add: (also eleborate more in the background section)
% OT: Peyré, M. Cuturi, Computational Optimal Transport, FNT in ML, 2019. -> \cite{peyre2019computational}
% Sinkhorn distance: 
% - Cuturi, Sinkhorn Distances: Lightspeed Computation of Optimal Transport, NIPS’13.  -> \cite{cuturi2013sinkhorn}
% - Séjourné et al., Sinkhorn Divergences for Unbalanced Optimal Transport, arXiv:1910.12958. -> \cite{sejourne2019sinkhorn}
% differtiable implementation:  ott-jax https://ott-jax.readthedocs.io/en/latest/ -> \cite{cuturi2021ott}

\subsection{Motivation of Our Work}

\todowriting{show the issue of works mathematically }
We want to improve the recent GAN (e.g. VQ-GAN) + CLIP line of work, 
such that it could contain more concepts (prompt) at the same time. 
Currently, the common practice is to let GAN generate an image that is close to the mean of CLIP embeddings of all concepts (prompts),


